Massive MIMO Beam Management in Sub-6 GHz 5G NR

Beam codebooks are a new feature of massive multiple-input multiple-output (M-MIMO) in 5G new radio (NR). Codebooks comprised of beamforming vectors are used to transmit reference signals and obtain limited channel state information (CSI) from receivers via the codeword index. This enables large arrays that cannot otherwise obtain sufficient CSI. The performance, however, is limited by the codebook design. In this paper, we show that machine learning can be used to train site-specific codebooks for initial access. We design a neural network based on an autoencoder architecture that uses a beamspace observation in combination with RF environment characteristics to improve the synchronization signal (SS) burst codebook. We test our algorithm using a flexible dataset of channels generated from QuaDRiGa. The results show that our model outperforms the industry standard (DFT beams) and approaches the optimal performance (perfect CSI and singular value decomposition (SVD)-based beamforming), using only a few bits of feedback.

==> IEEEabrv.tex <==
%%
%% IEEEabrv.bib
%%
%% BibTeX bibliography string definitions of the ABBREVIATED titles of
%% IEEE journals and magazines
%% 
%% NOTE: This text file uses MS Windows line feed conventions. When (human)
%% reading this file on other platforms, you may have to use a text
%% editor that can handle lines terminated by the MS Windows line feed
%% characters (0x0D 0x0A).
%%
%% This file is designed for bibliography styles that require 
%% abbreviated titles and is not for use in bibliographies that
%% require full-length titles.
%% 
%% Version 1.10 (2003/04/02)
%% 
%% Composed by Michael Shell
%% 
%% See:
%% http://www.ctan.org/tex-archive/macros/latex/contrib/supported/IEEEtran/
%% for latest version and current contact information.
%%
%% Special thanks to Laura Hyslop of IEEE for her help in obtaining the
%% information needed to compile this file. Also, Volker Kuhlmann kindly
%% provided some corrections and additions.
%%
%%**********************************************************************
%% Legal Notice:
%% This code is offered as-is without any warranty either expressed or
%% implied; without even the implied warranty of MERCHANTABILITY or
%% FITNESS FOR A PARTICULAR PURPOSE!
%% User assumes all risk.
%% In no event shall IEEE or any contributor to this code be liable for
%% any damages or losses, including, but not limited to, incidental,
%% consequential, or any other damages, resulting from the use or misuse
%% of any information contained here.
%%
%% This code is distributed under the Perl Artistic License 
%% ( http://language.perl.com/misc/Artistic.html ) 
%% and may be freely used, distributed and modified - subject to the
%% constraints therein.
%% Retain all contribution notices, credits and disclaimers.
%% 
%% All comments are the opinions of their respective authors and are not
%% necessarily endorsed by the IEEE.
%%**********************************************************************
%
%
% USAGE:
% 
% \bibliographystyle{mybstfile} 
% \bibliography{IEEEabrv,mybibfile}
%
% where the IEEE titles in the .bib database entries use the strings
% defined here. e.g.,
%
%
%    journal = IEEE_J_AC,
%
%
% to yield "{IEEE} Trans. Automat. Contr."
%
%
% IEEE uses abbreviated journal titles in their bibliographies -
% this file is suitable for work that is to be submitted to the IEEE.
%
%
% For work that requires full-length titles, you should use the full
% titles provided in the companion file, IEEEfull.bib.
%
%
% ** NOTES **
%
% 1. Journals have been grouped according to subject in order to make it
%    easier to locate and extract the definitions for related journals - 
%    as most works use references that are confined to a single topic.
%    Magazines are listed in straight alphabetical order.
%
% 2. String names are closely based on IEEE's own internal acronyms.
% 
% 3. Abbreviations follow IEEE's style.
%
% 4. Older, out-of-print IEEE titles are included (but not including titles
%    dating prior to IEEE's formation from the IRE and AIEE in 1963).
%
% 5. The following NEW/current journal definitions have been disabled because
%    their abbreviations have not yet been finalized/verified:
%    
%    STRING{IEEE_J_MC         = "{IEEE} Trans. Mobile Comput."}
%    STRING{IEEE_J_JEM        = "{IEEE/TMS} J. Electron. Mater."}
%    STRING{IEEE_J_MCTE       = "{IEEE} Trans. Molecular Cellular Tissue Eng."}
%    STRING{IEEE_J_ESSL       = "{IEEE/ECS} Electrochemical Solid-State Lett."}
%    STRING{IEEE_J_CJECE      = "Canadian J. Elect. Comput. Eng."}
%    
% 6. The following OLD journal definitions have been disabled because
%    their abbreviations have not yet been found/verified:
%
%    STRING{IEEE_J_EWS        = "{IEEE} Trans. Eng. Writing Speech"}
%    STRING{IEEE_J_BCTV       = "{IEEE} Trans. Broadcast Television Receivers"}
%
% If you know what the proper abbreviation is for a string in #5 or #6 above,
% email me and I will correct them in the next release.

%%%%%%%%%%%%%%%%%%%
%% Dates %%
%%%%%%%%%%%%%%%%%%%
@STRING{jan. = "Jan."}
@STRING{feb. = "Feb."}
@STRING{march = "March"}
@STRING{april = "April"}
@STRING{may = "May"}
@STRING{june = "June"}
@STRING{july = "July"}
@STRING{aug. = "Aug."}
@STRING{sep. = "Sep."}
@STRING{oct. = "Oct."}
@STRING{nov. = "Nov."}
@STRING{dec. = "Dec."}




%%%%%%%%%%%%%%%%%%%
%% IEEE Journals %%
%%%%%%%%%%%%%%%%%%%


% aerospace and military
@STRING{IEEE_J_AES        = "{IEEE} Trans. Aerosp. Electron. Syst."}
@STRING{IEEE_J_ANE        = "{IEEE} Trans. Aerosp. Navig. Electron."}
@STRING{IEEE_J_ANNE       = "{IEEE} Trans. Aeronaut. Navig. Electron."}
@STRING{IEEE_J_AS         = "{IEEE} Trans. Aerosp."}
@STRING{IEEE_J_AIRE       = "{IEEE} Trans. Airborne Electron."}
@STRING{IEEE_J_MIL        = "{IEEE} Trans. Mil. Electron."}



% autos, transportation and vehicles (non-aerospace)
@STRING{IEEE_J_ITS        = "{IEEE} Trans. Intell. Transport. Syst."}
@STRING{IEEE_J_VT         = "{IEEE} Trans. Veh. Technol."}
@STRING{IEEE_J_VC         = "{IEEE} Trans. Veh. Commun."}



% circuits, signals, systems, audio and controls
@STRING{IEEE_J_SPL        = "{IEEE} Signal Processing Lett."}
@STRING{IEEE_J_ASSP       = "{IEEE} Trans. Acoust., Speech, Signal Processing"}
@STRING{IEEE_J_AU         = "{IEEE} Trans. Audio"}
@STRING{IEEE_J_AUEA       = "{IEEE} Trans. Audio Electroacoust."}
@STRING{IEEE_J_AC         = "{IEEE} Trans. Automat. Contr."}
@STRING{IEEE_J_CAS        = "{IEEE} Trans. Circuits Syst."}
@STRING{IEEE_J_CASVT      = "{IEEE} Trans. Circuits Syst. Video Technol."}
@STRING{IEEE_J_CASI       = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII      = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CT         = "{IEEE} Trans. Circuit Theory"}
@STRING{IEEE_J_CST        = "{IEEE} Trans. Contr. Syst. Technol."}
@STRING{IEEE_J_SP         = "{IEEE} Trans. Signal Processing"}
@STRING{IEEE_J_SU         = "{IEEE} Trans. Sonics Ultrason."}
@STRING{IEEE_J_SAP        = "{IEEE} Trans. Speech Audio Processing"}
@STRING{IEEE_J_UE         = "{IEEE} Trans. Ultrason. Eng."}
@STRING{IEEE_J_UFFC       = "{IEEE} Trans. Ultrason., Ferroelect., Freq. Contr."}
@STRING{IEEE_J_JSTSP       = "{IEEE} J. Select. Topics Signal Processing"}



% communications
@STRING{IEEE_J_COML       = "{IEEE} Commun. Lett."}
@STRING{IEEE_J_JSAC       = "{IEEE} J. Select. Areas Commun."}
@STRING{IEEE_J_COM        = "{IEEE} Trans. Commun."}
@STRING{IEEE_J_COMT       = "{IEEE} Trans. Commun. Technol."}
@STRING{IEEE_J_WCOM       = "{IEEE} Trans. Wireless Commun."}



% components, packaging and manufacturing
@STRING{IEEE_J_ADVP       = "{IEEE} Trans. Adv. Packag."}
@STRING{IEEE_J_CHMT       = "{IEEE} Trans. Comp., Hybrids, Manufact. Technol."}
@STRING{IEEE_J_CPMTA      = "{IEEE} Trans. Comp., Packag., Manufact. Technol. {A}"}
@STRING{IEEE_J_CPMTB      = "{IEEE} Trans. Comp., Packag., Manufact. Technol. {B}"}
@STRING{IEEE_J_CPMTC      = "{IEEE} Trans. Comp., Packag., Manufact. Technol. {C}"}
@STRING{IEEE_J_CAPT       = "{IEEE} Trans. Comp. Packag. Technol."}
@STRING{IEEE_J_CAPTS      = "{IEEE} Trans. Comp. Packag. Technol."}
@STRING{IEEE_J_CPART      = "{IEEE} Trans. Comp. Parts"}
@STRING{IEEE_J_EPM        = "{IEEE} Trans. Electron. Packag. Manufact."}
@STRING{IEEE_J_MFT        = "{IEEE} Trans. Manufact. Technol."}
@STRING{IEEE_J_PHP        = "{IEEE} Trans. Parts, Hybrids, Packag."}
@STRING{IEEE_J_PMP        = "{IEEE} Trans. Parts, Mater., Packag."}



% CAD
@STRING{IEEE_J_TCAD       = "{IEEE} J. Technol. Computer Aided Design"}
@STRING{IEEE_J_CAD        = "{IEEE} Trans. Computer-Aided Design"}



% coding, data, information, knowledge
@STRING{IEEE_J_IT         = "{IEEE} Trans. Inform. Theory"}
@STRING{IEEE_J_KDE        = "{IEEE} Trans. Knowledge Data Eng."}



% computers, computation, networking and software
@STRING{IEEE_J_C          = "{IEEE} Trans. Comput."}
@STRING{IEEE_J_ECOMP      = "{IEEE} Trans. Electron. Comput."}
@STRING{IEEE_J_EVC        = "{IEEE} Trans. Evol. Comput."}
@STRING{IEEE_J_FUZZ       = "{IEEE} Trans. Fuzzy Syst."}
% disabled till definition finalized
STRING{IEEE_J_MC          = "{IEEE} Trans. Mobile Comput."}
@STRING{IEEE_J_NET        = "{IEEE/ACM} Trans. Networking"}
@STRING{IEEE_J_NN         = "{IEEE} Trans. Neural Networks"}
@STRING{IEEE_J_PDS        = "{IEEE} Trans. Parallel Distrib. Syst."}
@STRING{IEEE_J_SE         = "{IEEE} Trans. Software Eng."}



% computer graphics, imaging, and multimedia
@STRING{IEEE_J_IP         = "{IEEE} Trans. Image Processing"}
@STRING{IEEE_J_MM         = "{IEEE} Trans. Multimedia"}
@STRING{IEEE_J_VCG        = "{IEEE} Trans. Visual. Comput. Graphics"}



% cybernetics, ergonomics, robots, man-machine, and automation
@STRING{IEEE_J_JRA        = "{IEEE} J. Robot. Automat."}
@STRING{IEEE_J_HFE        = "{IEEE} Trans. Hum. Factors Electron."}
@STRING{IEEE_J_MMS        = "{IEEE} Trans. Man-Mach. Syst."}
@STRING{IEEE_J_PAMI       = "{IEEE} Trans. Pattern Anal. Machine Intell."}
@STRING{IEEE_J_RA         = "{IEEE} Trans. Robot. Automat."}
@STRING{IEEE_J_SMC        = "{IEEE} Trans. Syst., Man, Cybern."}
@STRING{IEEE_J_SMCA       = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
@STRING{IEEE_J_SMCB       = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
@STRING{IEEE_J_SMCC       = "{IEEE} Trans. Syst., Man, Cybern. {C}"}
@STRING{IEEE_J_SSC        = "{IEEE} Trans. Syst. Sci. Cybernetics"}



% earth, wind, fire and water
@STRING{IEEE_J_GE         = "{IEEE} Trans. Geosci. Electron."}
@STRING{IEEE_J_GRS        = "{IEEE} Trans. Geosci. Remote Sensing"}
@STRING{IEEE_J_OE         = "{IEEE} J. Oceanic Eng."}



% education, engineering, history, IEEE, professional
% disabled till definition is verified
STRING{IEEE_J_CJECE       = "Canadian J. Elect. Comput. Eng."}
@STRING{IEEE_J_PROC       = "Proc. {IEEE}"}
@STRING{IEEE_J_EDU        = "{IEEE} Trans. Educ."}
@STRING{IEEE_J_EM         = "{IEEE} Trans. Eng. Manage."}
% disabled till definition is verified
STRING{IEEE_J_EWS         = "{IEEE} Trans. Eng. Writing Speech"}
@STRING{IEEE_J_PC         = "{IEEE} Trans. Prof. Commun."}



% electromagnetics, antennas, EMI, magnetics and microwave
@STRING{IEEE_J_AWPL       = "{IEEE} Antennas Wireless Propagat. Lett."}
@STRING{IEEE_J_MGWL       = "{IEEE} Microwave Guided Wave Lett."}
% IEEE seems to want "Compon." here, not "Comp."
@STRING{IEEE_J_MWCL       = "{IEEE} Microwave Wireless Compon. Lett."}
@STRING{IEEE_J_AP         = "{IEEE} Trans. Antennas Propagat."}
@STRING{IEEE_J_EMC        = "{IEEE} Trans. Electromagn. Compat."}
@STRING{IEEE_J_MAG        = "{IEEE} Trans. Magn."}
@STRING{IEEE_J_MTT        = "{IEEE} Trans. Microwave Theory Tech."}
@STRING{IEEE_J_RFI        = "{IEEE} Trans. Radio Freq. Interference"}
@STRING{IEEE_J_TJMJ       = "{IEEE} Transl. J. Magn. Jpn."}



% energy and power
@STRING{IEEE_J_EC         = "{IEEE} Trans. Energy Conversion"}
@STRING{IEEE_J_PWRAS      = "{IEEE} Trans. Power App. Syst."}
@STRING{IEEE_J_PWRD       = "{IEEE} Trans. Power Delivery"}
@STRING{IEEE_J_PWRE       = "{IEEE} Trans. Power Electron."}
@STRING{IEEE_J_PWRS       = "{IEEE} Trans. Power Syst."}



% industrial, commercial and consumer
@STRING{IEEE_J_APPIND     = "{IEEE} Trans. Applicat. Ind."}
@STRING{IEEE_J_BC         = "{IEEE} Trans. Broadcast."}
% disabled till definition is verified
STRING{IEEE_J_BCTV        = "{IEEE} Trans. Broadcast Television Receivers"}
@STRING{IEEE_J_CE         = "{IEEE} Trans. Consumer Electron."}
@STRING{IEEE_J_IE         = "{IEEE} Trans. Ind. Electron."}
@STRING{IEEE_J_IECI       = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}
@STRING{IEEE_J_IA         = "{IEEE} Trans. Ind. Applicat."}
@STRING{IEEE_J_IGA        = "{IEEE} Trans. Ind. Gen. Applicat."}



% instrumentation and measurement
@STRING{IEEE_J_IM         = "{IEEE} Trans. Instrum. Meas."}



% insulation and materials
% disabled till definition finalized
STRING{IEEE_J_JEM         = "{IEEE/TMS} J. Electron. Mater."}
@STRING{IEEE_J_DEI        = "{IEEE} Trans. Dielect. Elect. Insulation"}
@STRING{IEEE_J_EI         = "{IEEE} Trans. Elect. Insulation"}



% mechanical
@STRING{IEEE_J_MECH       = "{IEEE/ASME} Trans. Mechatron."}
@STRING{IEEE_J_MEMS       = "J. Microelectromech. Syst."}



% medical and biological
@STRING{IEEE_J_BME        = "{IEEE} Trans. Biomed. Eng."}
% Note: The B-ME journal later dropped the hyphen and became the BME.
@STRING{IEEE_J_B-ME       = "{IEEE} Trans. Bio-Med. Eng."}
@STRING{IEEE_J_BMELC      = "{IEEE} Trans. Bio-Med. Electron."}
@STRING{IEEE_J_ITBM       = "{IEEE} Trans. Inform. Technol. Biomed."}
@STRING{IEEE_J_ME         = "{IEEE} Trans. Med. Electron."}
@STRING{IEEE_J_MI         = "{IEEE} Trans. Med. Imag."}
% disabled till definition finalized
STRING{IEEE_J_MCTE        = "{IEEE} Trans. Molecular Cellular Tissue Eng."}
@STRING{IEEE_J_NB         = "{IEEE} Trans. Nanobiosci."}
@STRING{IEEE_J_NSRE       = "{IEEE} Trans. Neural Syst. Rehab. Eng."}
@STRING{IEEE_J_RE         = "{IEEE} Trans. Rehab. Eng."}



% optics, lightwave and photonics
@STRING{IEEE_J_PTL        = "{IEEE} Photon. Technol. Lett."}
@STRING{IEEE_J_JLT        = "J. Lightwave Technol."}



% physics, electrons, nanotechnology, nuclear and quantum electronics
@STRING{IEEE_J_EDL        = "{IEEE} Electron Device Lett."}
@STRING{IEEE_J_JQE        = "{IEEE} J. Quantum Electron."}
@STRING{IEEE_J_JSTQE      = "{IEEE} J. Select. Topics Quantum Electron."}
@STRING{IEEE_J_ED         = "{IEEE} Trans. Electron Devices"}
@STRING{IEEE_J_NANO       = "{IEEE} Trans. Nanotechnol."}
@STRING{IEEE_J_NS         = "{IEEE} Trans. Nucl. Sci."}
@STRING{IEEE_J_PS         = "{IEEE} Trans. Plasma Sci."}



% reliability
% IEEE seems to want "Mat." here, not "Mater."
@STRING{IEEE_J_DMR        = "{IEEE} Trans. Device Mat. Rel."}
@STRING{IEEE_J_R          = "{IEEE} Trans. Rel."}



% semiconductors, superconductors, electrochemical and solid state
% disabled till definition finalized
STRING{IEEE_J_ESSL        = "{IEEE/ECS} Electrochemical Solid-State Lett."}
@STRING{IEEE_J_JSSC       = "{IEEE} J. Solid-State Circuits"}
@STRING{IEEE_J_ASC        = "{IEEE} Trans. Appl. Superconduct."}
@STRING{IEEE_J_SM         = "{IEEE} Trans. Semiconduct. Manufact."}



% sensors
@STRING{IEEE_J_SENSOR     = "{IEEE} Sensors J."}



% VLSI
@STRING{IEEE_J_VLSI       = "{IEEE} Trans. {VLSI} Syst."}





%%%%%%%%%%%%%%%%%%%%
%% IEEE Magazines %%
%%%%%%%%%%%%%%%%%%%%


@STRING{IEEE_M_AES        = "{IEEE} Aerosp. Electron. Syst. Mag"}
@STRING{IEEE_M_HIST       = "{IEEE} Annals Hist. Comput."}
@STRING{IEEE_M_AP         = "{IEEE} Antennas Propagat. Mag."}
@STRING{IEEE_M_ASSP       = "{IEEE} {ASSP} Mag."}
@STRING{IEEE_M_CD         = "{IEEE} Circuits Devices Mag."}
@STRING{IEEE_M_CAS        = "{IEEE} Circuits Syst. Mag."}
@STRING{IEEE_M_COM        = "{IEEE} Commun. Mag."}
@STRING{IEEE_M_COMSOC     = "{IEEE} Commun. Soc. Mag."}
% CSEM changed to CSE in 1999
@STRING{IEEE_M_CSE        = "{IEEE} Comput. Sci. Eng."}
@STRING{IEEE_M_CSEM       = "{IEEE} Comput. Sci. Eng. Mag."}
@STRING{IEEE_M_C          = "{IEEE} Computer"}
@STRING{IEEE_M_CAP        = "{IEEE} Comput. Appl. Power"}
@STRING{IEEE_M_CGA        = "{IEEE} Comput. Graph. Appl."}
@STRING{IEEE_M_CONC       = "{IEEE} Concurrency"}
@STRING{IEEE_M_CS         = "{IEEE} Control Syst. Mag."}
@STRING{IEEE_M_DTC        = "{IEEE} Des. Test. Comput."}
@STRING{IEEE_M_EI         = "{IEEE} Electr. Insul. Mag."}
@STRING{IEEE_M_EMB        = "{IEEE} Eng. Med. Biol. Mag."}
@STRING{IEEE_M_EMR        = "{IEEE} Eng. Manag. Rev."}
@STRING{IEEE_M_EXP        = "{IEEE} Expert"}
@STRING{IEEE_M_IA         = "{IEEE} Ind. Appl. Mag."}
@STRING{IEEE_M_IM         = "{IEEE} Instrum. Meas. Mag."}
@STRING{IEEE_M_IS         = "{IEEE} Intell. Syst."}
@STRING{IEEE_M_IC         = "{IEEE} Internet Comput."}
@STRING{IEEE_M_ITP        = "{IEEE} {IT} Prof."}
@STRING{IEEE_M_MICRO      = "{IEEE} Micro"}
@STRING{IEEE_M_MW         = "{IEEE} Microwave"}
@STRING{IEEE_M_MM         = "{IEEE} Multimedia"}
@STRING{IEEE_M_NET        = "{IEEE} Network"}
% IEEE's editorial manual lists "Pers. Commun.", 
% but "Personal Commun. Mag." seems to be what is used in the journals
@STRING{IEEE_M_PCOM       = "{IEEE} Personal Commun. Mag."}
@STRING{IEEE_M_POT        = "{IEEE} Potentials"}
% CAP and PER merged to form PE in 2003
@STRING{IEEE_M_PE         = "{IEEE} Power Energy Mag."}
@STRING{IEEE_M_PER        = "{IEEE} Power Eng. Rev."}
@STRING{IEEE_M_RA         = "{IEEE} Robot. Automat. Mag."}
@STRING{IEEE_M_SP         = "{IEEE} Signal Processing Mag."}
@STRING{IEEE_M_S          = "{IEEE} Softw."}
@STRING{IEEE_M_SPECT      = "{IEEE} Spectr."}
@STRING{IEEE_M_TS         = "{IEEE} Technol. Soc. Mag."}
@STRING{IEEE_M_WC         = "{IEEE} Wireless Commun. Mag."}
@STRING{IEEE_M_TODAY      = "Today's Eng."}




%--
%EOF

